Digging Errors in NMT: Evaluating and Understanding Model Errors from Partial Hypothesis Space

Solid evaluation of neural machine translation (NMT) is key to its understanding and improvement. Current evaluation of an NMT system is usually built upon a heuristic decoding algorithm (e.g., beam search) and an evaluation metric assessing similarity between the translation and golden reference. However, this system-level evaluation framework is limited by evaluating only one best hypothesis and search errors brought by heuristic decoding algorithms. To better understand NMT models, we propose a novel evaluation protocol, which defines model errors with model's ranking capability over hypothesis space. To tackle the problem of exponentially large space, we propose two approximation methods, top region evaluation along with an exact top-$k$ decoding algorithm, which finds top-ranked hypotheses in the whole hypothesis space, and Monte Carlo sampling evaluation, which simulates hypothesis space from a broader perspective. To quantify errors, we define our NMT model errors by measuring distance between the hypothesis array ranked by the model and the ideally ranked hypothesis array. After confirming the strong correlation with human judgment, we apply our evaluation to various NMT benchmarks and model architectures. We show that the state-of-the-art Transformer models face serious ranking issues and only perform at the random chance level in the top region. We further analyze model errors on architectures with different depths and widths, as well as different data-augmentation techniques, showing how these factors affect model errors. Finally, we connect model errors with the search algorithms and provide interesting findings of beam search inductive bias and correlation with Minimum Bayes Risk (MBR) decoding.

==> edit_distance.tex <==
\section{Edit-Distance-based Evaluation}
\label{sec:edit-dist}
% move above 
% Even with the truncated $\tilde{P}$, it is non-trivial to evaluate model's outputs using just the references. 
% As for HR distribution, 
% The difficulty mainly comes from the unawareness of global model distribution.
% use the marginal reward distribution to evaluate the top ranked outputs.
In this section, we provide an approach for computing model errors, which do not rely on approximation for $\bm{\mathcal{Y}_{\text{HR}}}$.
% Here, we do not want to approximate $\bm{\mathcal{Y}_{\text{HR}}}$.
The challenge is to score the unbounded hypothesis space . It would be helpful if a HR array with a certain translation quality function $Q$ can be queried without actually constructing the array.

Therefore, inspired by \citep{norouzi2016reward}, we model $\bm{\mathcal{Y}_{\text{HR}}}$ with an edit-distance based ranked array, where each hypothesis is ranked by its edit-distance to the references,
\begin{gather}
    Q(y_i, \hat{y}, x) = -\text{Edit\_Distance}(y_i, \hat{y}),
\end{gather}
where a larger edit distance means a lower rank in the HR array.
Then, given a hypothesis $y_i$ with $e$ edits to reference, we can predict the number of hypotheses with $e$ edits from $\hat{y}$ by,
\begin{gather}
    c(e, T) = \sum_{s=0}^T \binom{T}{s} \binom{T+e-2s}{e-s} |V|^e, 
\end{gather}
where $s$ is the number of substitution operations and $|V|$ is the vocabulary size. 
For more details, we refer our readers to \citep{norouzi2016reward}.
Then we can estimate the rank of a hypothesis $y_i$ with the sum of numbers of hypotheses with edit distance lower than $e$,
\begin{gather}
    \text{Rank}(y) = \sum_{e'\in[0, e)} c(e', T).
\end{gather}
The visualization of edit-distance rankings is shown in Figure \ref{fig:global}, which illustrates how the model error changes when using different architectures and techniques. 

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
        \centering
        \includegraphics[width=\linewidth]{img/trans_hist.pdf}
        \caption[Network2]%
        {{\small Loss and pseudo data.}}    
        \label{fig:mean and std of net14}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.245\linewidth}  
        \centering 
        \includegraphics[width=\linewidth]{img/dropout_hist.pdf}
        \caption[]%
        {{\small Different dropouts.}}    
        \label{fig:mean and std of net24}
    \end{subfigure}
    % \vskip\baselineskip
    \begin{subfigure}[b]{0.245\linewidth}   
        \centering 
        \includegraphics[width=\linewidth]{img/deeper_hist.pdf}
        \caption[]%
        {{\small Deeper architectures.}}    
        \label{fig:mean and std of net34}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.245\linewidth}   
        \centering 
        \includegraphics[width=\linewidth]{img/wider_hist.pdf}
        \caption[]%
        {{\small Wider architectures.}}    
        \label{fig:mean and std of net44}
    \end{subfigure}

    \caption[]
    {The edit-distance ranking visualization of Transformer models with different techniques. Here, we use top-$10$ hypotheses of exact search. \textbf{para FT} and \textbf{para BT} denote the model trained with both golden dataset and forward/backward generated pseudo dataset. } 
    \label{fig:global}
\end{figure*}

Note that we use exact top-$100$ hypotheses of model distribution for this visualization. We expect the hypotheses are located among the top $0\sim 10\%$ of edit-distance rankings.
Interestingly, across all models, the probability mass of these top-ranking hypotheses lies either in the top $10\%$ or the last $10\%$ of edit-distance ranks.
About $70\%$ of the hypotheses are located in the last $10\%$. 
It indicates model errors are severe, where the model prefers both good hypotheses (ranked $0\sim 10\%$) and bad hypotheses (ranked $90\% \sim 100\%$). 
In addition, we make several observations:
\begin{itemize}
    \item A model without label smoothing strongly decreases the number of top hypotheses in the last $10\%$ of ranks. (Figure \ref{fig:global}(a))
    \item Pseudo data generation techniques decrease the model errors. The model with forward-translated data significantly decreases model errors. (Figure \ref{fig:global}(a))
    \item Increasing the dropout rate does not necessarily improve model errors. (Figure \ref{fig:global}(b))
    \item Increasing model capacity, like deepening or widening model architectures, generally reduces model errors monotonically. (Figure \ref{fig:global}(c, d))
\end{itemize}

We use edit-distance metric because the commonly used metrics in NMT (e.g., BLEU or METOR) are difficult to estimate the ranks of hypotheses, therefore cannot provide the above analysis. 

\section{Investigations on Beam Search Curse}

Our proposed exact top-$k$ decoding algorithm enables us to investigate the relationship between the beam search algorithm and the top-$k$ decoding algorithm. First, we conduct an experiment to help understand to what extent these two algorithms disagree. We first run the exact decoding algorithm using $k=100$ and beam search with beam sizes of 5, 10, 20, 50, 100 on the WMT' 14 English-German testset. We plot the ranked positions of the beam search results over the exact outputs in Figure \ref{fig:beam_ranks}, which demonstrates that a larger beam size leads to fewer search errors since the ranked positions of those hypotheses are higher. However, the BLEU scores of the beam search results are inversely proportional to the beam size, which are $27.28\%, 27.27\%, 26.98\%, 26.03\%, 23.87\%$ respectively. This is called \emph{beam search curse} \citep{yang2018breaking} - translation quality degrades as beam sizes increases.

\begin{figure}
\centering
\begin{subfigure}[t]{0.45\linewidth}
% \begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/beam_ranks.pdf}
    \caption[Network2]
    {{\small}}
    \label{fig:beam_ranks}
\end{subfigure}
% \begin{subfigure}[t]{0.45\linewidth}
% % \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{img/bleu_scores.pdf}
%     \caption[Network2]
%     {{\small }}
% %    \chenming{Change `100' to `>100' later on}}
%     \label{fig:bleu_scores}
% % \end{figure}
% \end{subfigure}
\begin{subfigure}[t]{0.45\linewidth}
% \begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/random_change.pdf}
    \caption[Network2]
    {{\small }}
%    \chenming{Change `100' to `>100' later on}}
    \label{fig:random_change}
% \end{figure}
\end{subfigure}
\caption{The experimental results of comparing top-$k$ exact decoding with beam search decoding. (a) The numbers of ranked positions of different beam search results. (b) Sentence-level BLEU trends when increasing the beam size. The horizontal axis is the number of changes (positive values means getting better, vice versa). The vertical axis is the counts of changes.}
%: each sentence use its BLEU of the result using beam size 5 as a baseline. `\#Change' means the count of improved (positive) or decreased (negative) BLEU using the other beam sizes (i.e., 10, 20, 50, 100). \elliott{no description of what x, y are.}
\end{figure}

We further investigate the trends in terms of BLEU scores from sentence-level when using a larger beam size. For each source sentence, we track the BLEU score of its translated sentence from a small beam size to a large beam size. As a result, we can obtain two properties for each sentence. One is the number of getting a better translation. Conversely, the other is the number of getting a worse translation. We plot the results in Figure \ref{fig:random_change}. The results show that the trend is random in sentence-level, and not consistent with the facts we observe from the whole dataset.
This reveals that the NMT model has a large number of ranking errors, i.e., two very close hypotheses may be ordered falsely by the model.

Based on the above experimental results, we discover that \emph{beam search curse} is closely related to the \textbf{hypothesis ranking} of an NMT model. This finding motivates us to study how to evaluate the hypothesis distribution of an NMT system.
If an NMT model can successfully order all hypotheses by a certain scoring function, the \emph{beam search curse} will disappear. 


==> min_heap.tex <==
\section{Approximate Exact Decoding}
% \section{Min-heap Beam Search} 
The ranking-based ME enables us to evaluate the quality of NMT models and find new problems from a different perspective. 
A fact is that the algorithm of an evaluation protocol should be consistent with the algorithm used in production. For instance, the beam search with BLEU evaluation protocol is widely used because beam search is commonly adopted in production. Otherwise, the evaluation is hard to provide informative clues for improving the quality of production models. Nevertheless, our proposed ME relies on the proposed exact top-$k$ decoding, and the exact decoding methods are still far from the beam search decoding with regard to the computational cost. We argue that the future of sequence decoding should be either a super-fast exact decoding approach or an approximate algorithm that decodes as close as exact algorithms. In this section, we propose a solution based on beam search to approximate exact algorithms while not sacrificing computational time.

Beam search is an improved version of greedy algorithm, it uses a limited breadth $b\in \mathcal{Z}_+$ to prune breadth-first search (BFS) algorithm. Specifically, at each step of expansion, only $b$ best candidates are stored and others are pruned. We follow the notations defined in Section 4 here. The target of beam search decoding is to find a target sentence $y^*=\arg\max \log P(y \mid x)$ overall all candidate sets. Let $\mathbf{Y}_t$ be the prioritized hypothesises at step $t$, then it can be expressed as:
\begin{gather} 
    \mathbf{Y}_0 = \{\rm BOS\} \\
    \mathbf{Y}_t = \arg{\rm{top}_b} \{\log P(y^t_i \mid x) \mid y_i \in \mathbf{B}_t\}
\end{gather}
where $\mathbf{B}_t$ denotes all candidates from which beam search can select, and it can be defined as:
\begin{gather}
    \mathbf{B}_t = \{y^{t-1}_i \circ v \mid y^{t-1}_i \in \mathbf{Y}_{t-1}, v\in V\}
\end{gather}
Beam search terminates after a predefined number of iterations, or if all candidates end with $\rm EOS$, or satisfying a specific early-stopping criterion. The output of beam search is $\mathbf{Y}_T$ where $T$ is the end time step. The design philosophy of beam search algorithm discards candidate $y_t$ with the following form on purpose:
\begin{gather}
    y^{t}_i = \{ y^{t-1}_i \circ {\rm EOS} \}  \: \text{and} \: y^t_i \not\in \mathbf{Y}_{t},
\end{gather}
where $\circ$ denotes string concatenation. The above case often happens at the beginning of decoding; that is, an empty sentence $y_{emp}$'s score is overall the highest, but it is pruned because it is worse than the chosen $k$ candidates. This explains why many empty sentences are not captured by beam search algorithm but count for the most percentage by \citep{stahlberg-byrne-2019-nmt}.

We make a simple yet effective modification to the original beam search algorithm by adding a minimum heap $H$. The capacity of $H$ is identical to the beam size. Unlike the original beam search, we propose to push all candidates in $\mathbf{B}_t$ end with $\rm EOS$ to $H$. When beam search terminates, we replace the output $\mathbf{Y}_T$ of beam search with $H$ as the final output. 

\textbf{Theorem:} The target sentences in $H$ are not worse than the target sentences in $\mathbf{Y}_T$.

\begin{proof} 
If there exists a sentence $\bar{y} \in \mathbf{Y}_T$ which has a better score than any sentence in $H$, its score must be lower than the minimum score of $H$. However, the minimum score of $H$ is monotonically increased.
\end{proof} 


\begin{table}
\centering
% \resizebox{0.8\columnwidth}{!}{%
\setlength\tabcolsep{2pt}
\captionof{table}{Search error statistics for beam search, min-heap beam search, and exact search in WMT'14 En-De task. All numbers range in [0, 100\%.}
\label{table:search_err}
\begin{tabular}{l||c || c  || c}
% \small
\toprule
{\bf Method} & \bf Beam Search ($\downarrow$)&\bf Min-heap Beam Search ($\downarrow$) & \bf Exact Search \\
\midrule
Transformer(base) & 67.53\% & 2.20\% & 0 \%\\
\midrule
\quad - label smoothing & 48.01\% & 12.49\% & 0 \%\\
\quad + para ft & 4.10\% & 3.03\% & 0 \% \\
%\quad + para bt & \% & \% & 0 \% \\
%\quad + dropout 0.2 & 65.0\% & \% & 0 \% \\
%\quad + dropout 0.3 & 63.0\% & \% & 0 \% \\
\midrule
Transformer(Dim 768) & 57.61\% & 6.13\% & 0 \%\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
% \resizebox{0.8\columnwidth}{!}{%
\setlength\tabcolsep{2pt}
\captionof{table}{BLEU scores of beam search and our min-heap beam search using different regularization terms in WMT'14 En-De task. All numbers range in [0, 100].}
\label{table:bleu_min_heap}
\begin{tabular}{l||c || c  }
% \small
\toprule
{\bf Method} & \bf Beam Search &\bf Min-heap Beam Search \\
\midrule
Transformer(base) & 27.22 & 0.40  \\
\midrule
% \bf Metric & BLEU & BLEU & BLEU \\
\quad + length normalization & 26.72 & 26.73 \\
\quad + greedy regularization & 27.38 & 27.36  \\
\quad + max regularization & 27.44 & 26.18 \\
\quad + square regularization & 27.43 & 27.21 \\
\quad + variance regularization & 27.35 & 26.37 \\
\bottomrule
\end{tabular}
\end{table}

We conduct an experiment to compare the search errors using the definition proposed in \citep{stahlberg-byrne-2019-nmt}. Table \ref{table:search_err} shows the results that the percentage of exact matched sentences is significantly increased compared to the ones of original beam search. The results empirically demonstrate that our proposed min-heap beam search approximates exact search decoding well.

We conduct an additional experiment on comparing search regularization terms (see Table \ref{table:bleu_min_heap}). Exact decoding is impossible to achieve since the regularization usually makes the scoring function non-monotonic. Thus we use the proposed min-heap beam search to investigate this problem. The experimental results show that length normalization and greedy regularization might be more suitable for NMT compared to other regularization techniques.

Min-heap beam search is an efficient approximation to the exact decoding, and it is effortlessly to replace beam search with min-heap beam search. There are many unknown areas to explore by revisiting previously proposed techniques using the min-heap beam search as an approximation, such as schedule sampling \citep{zhang-etal-2019-bridging}, reinforcement-learning-based training \citep{wu-etal-2018-study}, and so on.


==> search_errors.tex <==
\section{Search Errors}
The MAP decoding targets on finding the best candidate measured by accumulative log-probabilities, which has been widely used in modern NMT systems. However, this approach suffers from the exponential search space because NMT systems normally have a large vocabulary. As a result, beam search decoding is a popular technique to tackle this problem, which only stores a few candidates during the whole period of expansion. Pruning possible candidates results in errors between the produced results and the best results. Besides, different strategies between the training phase and decoding phase (i.e., autoregressive property) also lead to search errors. In this section, we propose a more formally way to describe the errors appeared in the decoding phase, and make a comprehensive analysis based on the experimental results.

The correctness of evaluating the search errors depends on the computation of dissimilarity between ground-truth and search results. Previous methods such as \citep{x} use the percentage of exact matched pairs between the DFS top-1 and the best result produced by beam search algorithms. This metric is easy to implement and works well for many cases. However, the design of this metric has limitation as it is not correlated with the autoregressive property, as the autoregressive decoding works on token-level and from one side to the other side. Exact matching only care if two sentences are identical. Therefore, easy to fail on certain circumstances.

For example, we use the exact matching metric to evaluate the search errors of transformer big model equipped with different beam search strategies. The experiment is conducted on WMT English-Germany 14 as well. 

\subsection{The definition of SE}

\textbf{SE on Models}

\textbf{SE on Decoding}

different divisions

different length - se

\subsection{Relation to Confidence}
para-ft no lb

\subsection{Fix Beam Search with Min-Heap}
analysis

